R+R: Revisiting Static Feature-Based Android Malware Detection using Machine Learning

Static feature-based Android malware detection using machine learning (ML) remains critical due to its scalability and efficiency. However, existing approaches often overlook security-critical reproducibility concerns, such as dataset duplication, inadequate hyperparameter tuning, and variance from random initialization. This can significantly compromise the practical effectiveness of these systems. In this paper, we systematically investigate these challenges by proposing a more rigorous methodology for model selection and evaluation. Using two widely used datasets, Drebin and APIGraph, we evaluate six ML models of varying complexity under both offline and continuous active learning settings. Our analysis demonstrates that, contrary to popular belief, well-tuned, simpler models, particularly tree-based methods like XGBoost, consistently outperform more complex neural networks, especially when duplicates are removed. To promote transparency and reproducibility, we open-source our codebase, which is extensible for integrating new models and datasets, facilitating reproducible security research.

==> sections-old/adv_attack.tex <==
\section{Adversarial Robustness}
We evaluate a pure black-box, score-based, feature-space evasion~\cite{simonetto2024constrained} on APIGraph and Drebin datasets. The Constrained Adaptive Attack (CAA) is a state-of-the-art method for adversarial evasion on tabular data that combines a fast gradient-based phase (CAPGD) with a stronger search phase. In our setting, we disable CAPGD and use only the search phase: a best-first beam search over single-bit add-only flips that batch-queries model scores, retains the lowest-score successors in a fixed-width beam (width 16; node cap 64), and halts upon reaching the benign threshold, exhausting the flip budget, or hitting the node cap. The attacker may flip up to \(B\) binary features per sample under an add-only constraint; all features are treated as mutable. We attack 500 randomly sampled malware test points per model, while benign samples remain unchanged.

Results are shown in Figure~\ref{fig:asr} for budgets \(B \in \{1,2,3,4,5\}\). Even with small budgets, the attack achieves high success across all models. On APIGraph, XGBoost and HCC are more robust than MLP, whereas on Drebin, XGBoost shows higher ASR than MLP for larger budgets (\(B=3,4,5\)), indicating that higher clean accuracy does not necessarily imply stronger adversarial robustness.



\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\linewidth]{figures/asr_apigraph.pdf}
    \hfill
    \includegraphics[width=0.48\linewidth]{figures/asr_drebin (1).pdf}
    \caption{Comparison of attack success rate .}
    \label{fig:asr}
\end{figure}











==> sections-old/background.tex <==
\section{Background \& Related Work}

\begin{table*}[t]
\caption{Summary statistics of the datasets used in the study}
\centering

\begin{tabular}{@{}cccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Split} & \textbf{Duration} & \textbf{\begin{tabular}[c]{@{}c@{}}Benign \\ Apps\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Malicious\\ Apps\end{tabular}} & \textbf{Total} & \textbf{\begin{tabular}[c]{@{}c@{}}Malware\\ Families\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}c@{}}Feature\\ Dimension\end{tabular}}} \\ \toprule
\multirow{3}{*}{Drebin} & Train & 2019-01 to 2019-12 & 40,947 & 4,542 & 45,489 & 121 & \multirow{3}{*}{16,978} \\
 & Validation & 2020-01 to 2020-06 & 18,109 & 2,028 & 20,137 & 67 &  \\
 & Test & 2020-07 to 2021-12 & 30,797 & 3,631 & 34,428 & 71 &  \\ \midrule
\multirow{3}{*}{APIGraph} & Train & 2012-01 to 2012-12 & 27,472 & 3,061 & 30,533 & 104 & \multirow{3}{*}{1,159} \\
 & Validation & 2013-01 to 2013-06 & 21,310 & 2,366 & 23,676 & 115 &  \\
 & Test & 2013-07 to 2018-12 & 240,729 & 25,377 & 266,106  & 418 &  \\ \bottomrule
\end{tabular}


\label{tab:datasets}
\end{table*}


\subsection{Reproducibility \& Replicability}

We adhere to ACM's definitions of reproducibility and replicability, standardized in 2020.\footnote{\url{https://www.acm.org/publications/policies/artifact-review-and-badging-current}}. Computational reproducibility refers to the ability of an independent team to achieve a study's results using the original study's artifacts~\cite{gundersen2018state}. This ensures that the reported findings are valid under specified conditions.~\cite{olszewski2023get} conducted a longitudinal study on the reproducibility of security papers published in Tier 1 venues (2013-2022), identifying challenges in reproducing results with author-provided artifacts and proposing mitigation strategies.

Replicability, in contrast, implies that an independent group can obtain the same results using artifacts they develop independently. Replicability studies generally involve different datasets and aim to confirm previous research results, considering the underlying system's inherent uncertainty.

Our study examines both aspects of machine learning research for Android malware detection. For instance, the analysis shown in Figure~\ref{fig:hcc-best-worst} underscores reproducibility issues in prior research, even when author-provided artifacts are used, due to unaccounted variability in published results. Additionally, we discuss pitfalls that must be addressed for a study's claims to be replicable with independently developed artifacts. In this paper, we use the term reproducibility to broadly refer to both computational reproducibility and replicability.  


%While previous works have analyzed ML design and datasets in security~\citep{arp2022and, flood2024bad, verma2019data, sculley2018winner}, there is limited research on enhancing the replicability of ML results for malware detection.




% \cite{arp2022and} identified pitfalls in the data collection and labeling, system design, implementation, performance evaluation and deployment of machine learning security in 30 papers from top-tier security conferences and suggested actionable recommendations to mitigate the pitfalls. %\cite{flood2024bad} study seven highly cited network intrusion dataset and discover that these dataset suffer from poor data diversity, highly dependent features, unclear ground truth, traffic collapse, artificial diversity and wrong labels. \cite{verma2019data} also discusses data quality in phishing, malware and intrusion detection datasets.%\cite{sculley2018winner} Perform a meta-analysis on several machine learning papers and found evidences of lack of rigorous standards for empirical work. 


\subsection{Android Malware Detection}

Android malware detection using machine learning classifies applications as benign or malicious~\cite{liu2020review}. Three main types of features are used: static, dynamic, and hybrid. Static features are obtained by analyzing the app's source code or related information~\cite{arp2014drebin,mamadroid,zhang2020enhancing}. Specifically, the primary focus for Android applications is the APK file, the installation package, which includes components like AndroidManifest.xml and smali files obtained through decompilation. Dynamic features are acquired by observing the app's behavior in real or emulated environments, such as sandboxes~\cite{jannat2019analysis,shankar2017androtaint,zhang2018dalvik}. Hybrid features combine both static and dynamic characteristics~\cite{choudhary2018haamd,martinelli2017bridemaid}. 

Extracted features are input into machine learning models like Random Forests~\cite{breiman2001random}, Support Vector Machines~\cite{arp2014drebin}, and Multilayer Perceptrons~\cite{rumelhart1986learning} to classify apps as malware or benign. The choice of features and models depends on detection objectives and resources. Static analysis is fast and suitable for large-scale detection, whereas dynamic analysis can be more accurate but resource-intensive~\cite{aghakhani2020malware}. This work focuses on static-feature-based machine learning methods due to their prevalence in the literature~\cite{ jordaney2017transcend, pendlebury2019tesseract, zhang2020enhancing, barbero2022transcending, chen2023continuous}. 




\textbf{Concept Drift:} Malware detection systems encounter challenges due to the evolving nature of malware, leading to concept drift. This drift can arise from new malware families, behavioral changes, evasion attempts, or updates in API semantics. Traditional supervised learning models trained on static datasets may become outdated as new malware types emerge, reducing detection accuracy~\cite{yang2021cade,chow2023drift,pendlebury2019tesseract,xu2019droidevolver}. These models often fail to recognize emerging variants, resulting in higher false negatives. To address this, continuous learning methods can enable models to adapt to new data continuously and stay current with malware trends~\cite{jordaney2017transcend,chen2023continuous}.


\textbf{Reproducibility of Research in Android Malware Detection Using ML:} Previous studies have assessed issues in reported results for Android malware detection~\cite{zhao2021impact,irolla2018duplication}, attempted to replicate prior research~\cite{daoudi2021lessons}, or addressed limitations in practical environments~\cite{gao2024comprehensive}. However, these studies do not consider the continuous learning setup, often rely on single global metrics like AUC or F1-score, lacking nuanced analysis of monthly performance variations, factors influencing reproducibility, and inherent variances in machine learning models due to their stochastic nature. Our work aims to address these gaps by analyzing conditions that can lead to poor reproducibility in different experimental settings and how to mitigate them.




\section{Study settings}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\subsection{Machine Learning Scenarios}
We evaluate Android malware detection models under 2 distinct ML scenarios relevant to practical security deployment:

\begin{enumerate}
    \item \textbf{Offline Learning:} Models are trained once on the historical dataset and then evaluated on unseen future data, reflecting static deployment scenarios. This involves using annotated data from a specific period (e.g., one year) to train a model.

    \item \textbf{Continuous Active Learning:} To address the evolving nature of malware (concept drift), we periodically retrain the model~\cite{jordaney2017transcend,zhang2020enhancing,chen2023continuous} using only the samples where the model is least confident, saving annotation resources. We adopt monthly retraining intervals, consistent with established literature.
    % This provides a standard evaluation setting for active learning methods independent of drift detection techniques. 
    %We adopt this approach in our study.
\end{enumerate}

We treat these settings separately because each requires different model selection methods, such as hyperparameter tuning, as noted in prior work~\cite{chen2023continuous}. 
% We aim to analyze the factors influencing replicability in these settings and enhance the reliability of Android malware detection models.



\subsection{Datasets}

We utilize the publicly available dataset from~\cite{chen2023continuous}, which includes two datasets based on static feature types: Drebin~\cite{arp2014drebin} and APIGraph~\cite{zhang2020enhancing}. Hereafter, we refer to these as the Drebin and APIGraph datasets. Drebin uses eight different sets of features, including access to hardware components, requested permissions, app components, intents, usage of restricted API calls, used permissions, suspicious API calls, and network addresses. APIGraph employs API semantics to cluster similar APIs, significantly reducing the feature space. The resulting feature set is binary for both datasets, indicating whether a feature is present or absent for a specific sample.

The Drebin dataset contains applications collected from 2019 to 2021, while the APIGraph dataset includes applications from 2012 to 2018. Both datasets address temporal and spatial biases present in malware datasets~\cite{arp2022and, pendlebury2019tesseract}. They consist of approximately 90\% benign and 10\% malware applications collected from each month, reflecting their real-world ratios. Samples are ordered and approximately evenly distributed over their respective periods. Table~\ref{tab:datasets} provides a summary of the datasets.

Following~\cite{chen2023continuous}, we use data from the first year as the training set, the next six months for validation, and the remaining months for testing. For offline learning, only the training set data is used to train the model. In the continuous active learning setup, this data is used to train the initial model, which is then periodically retrained using data from subsequent months from the validation and test set. The validation set is used to tune the model hyperparameters in both experimental settings. 




==> sections-old/conclusion.tex <==
\section{Conclusion}

In this paper, we systematically revisited critical reproducibility and replicability challenges in static feature-based Android malware detection using machine learning. We focus on key pitfalls in dataset curation, model selection, and evaluation strategies. Our extensive evaluation across multiple machine learning models in offline and continuous active learning settings reveals that common yet overlooked issues, such as data duplication, inadequate hyperparameter tuning, and biased model selection, can lead to significant performance disparities, significantly undermining the security and reliability of detection systems. These findings highlight the need for more rigorous approaches to ensure the reliability of reported results. Our results indicate that, with proper tuning, simpler models can often match or surpass the performance of more complex methods, challenging the trend of relying solely on sophisticated architectures. %To support future research, we provide detailed recommendations to enhance reproducibility in Android malware detection using ML, many of which can also be applied to other security tasks. 
Our open-source code offers a standardized, extensible framework for benchmarking new models, facilitating fairer and more reliable comparisons across studies. %By making our framework available, we aim to contribute to a more transparent and robust research environment, thereby enhancing the reproducibility of future work in this field. 





\clearpage


% \section*{Ethics consideration}

% Our paper addresses critical issues related to reproducibility and replicability in Android malware detection. Given the potential impact of our findings and methods, several ethical considerations were carefully reviewed to ensure alignment with community standards and broader ethical principles.

% \begin{enumerate}
%     \item \textbf{Beneficence:} Our research utilizes Android application datasets that do not include sensitive personal information. It is crucial to recognize that improvements in malware detection systems enhance user security. Our methods are designed to improve the safety of software ecosystems without harming individual stakeholders. We ensure that no sensitive user data is collected, maintaining privacy and ethical standards.

%     \item \textbf{Justice:} We have made our code open-source to promote transparency, reproducibility, and opportunities for others to build upon our work, fostering fairness in the research community and enabling equitable access to improved malware detection systems.

%     \item \textbf{Respect for Law and Public Interest:} All datasets used in this study are publicly available and utilized according to their terms. No Terms of Service were violated, and no deceptive methods were employed during experimentation or evaluation.

%     \item \textbf{Potential Negative Impacts:} We acknowledge that both defenders and adversaries can use improvements in malware detection. While our work aims to enhance defensive strategies, effective detection techniques could be reverse-engineered by malicious actors. We adhere to responsible disclosure principles to mitigate this and use only well-documented, publicly available datasets without exposing new vulnerabilities.

% \end{enumerate}

% \section*{Open science policy}

% We are committed to fostering open science by sharing all research artifacts necessary for reproducing and extending the findings of this study. Our primary focus is ensuring that future researchers can validate our results, replicate our methodologies, and build upon our work to advance the field of Android malware detection. We openly provide the following artifacts:

% \begin{enumerate}
%     \item \textbf{Source Code:} All the source code used in our experiments, including implementations of the machine learning models, active learning methods, and evaluation scripts, will be made publicly available upon publication. The code is well-documented and organized to facilitate ease of use and extension for future research.
    
% \item \textbf{Datasets:} We used publicly available Android malware datasets which are openly accessible. These datasets are used within their licensing terms, and we include references to the sources so that others can obtain and use the same data. 

% \item \textbf{Scripts and Configuration Files:} In addition to the code, we provide the configuration files, hyperparameter settings, and detailed instructions for running the experiments. This includes the exact settings used to replicate the results reported in our paper, such as different random seed initializations and model hyperparameters.
% \end{enumerate}

% Our artifact repository is currently available at \url{https://anonymous.4open.science/r/revisiting-static-mal/}. We are committed to maintaining this repository to ensure the artifacts remain accessible and functional for the research community.

% If any issues related to dataset licensing arise, we will provide detailed justifications and work with the Artifact Evaluation committee to find suitable solutions. However, at present, we anticipate no such restrictions.

% In conclusion, the ethical implications of this research were considered across various frameworks, and we believe that the positive outcomes, particularly in enhancing reproducibility in security research, significantly outweigh any potential negative consequences. We remain committed to following best practices in ethical research to promote security and trust in the malware detection community.

==> sections-old/experiments.tex <==
\section{Experiments}






\subsection{Machine Learning Models}

We utilize six different models commonly used in prior works on Android malware detection:

\begin{enumerate}
\item \textbf{Random Forest (RF):} Random Forest~\cite{breiman2001random} is an ensemble learning method for classification that constructs multiple decision trees during training and outputs the mode of their classes. It has been used in Android malware detection~\cite{sanz2013puma,mamadroid}.

\item \textbf{Support Vector Machine (SVM):} SVM~\cite{cortes1995support} is a classification algorithm that finds the hyperplane that best separates classes in the feature space. It has been widely used for Android malware detection, particularly with Drebin features~\cite{arp2014drebin,jordaney2017transcend}.

\item \textbf{eXtreme Gradient Boosting (XGBoost):} XGBoost~\cite{chen2016xgboost} is a scalable and efficient gradient boosting method that excels in performance on various tabular datasets~\cite{grinsztajn2022tree}, although it has not shown consistent success in Android malware detection~\cite{chen2023continuous}.

\item \textbf{Multilayer Perceptron (MLP):} An MLP is a type of neural network composed of multiple layers of neurons, with each layer fully connected to the next~\cite{rumelhart1986learning}. MLPs are used for a variety of tasks, including classification and regression, and have been employed in several prior works for Android malware detection~\cite{pendlebury2019tesseract,yuan2016droiddetector,kim2018multimodal}.


\item \textbf{Supervised Contrastive Classifier (SCC):} Contrastive learning effectively detects and adapts to concept drift in Android malware detection~\cite{yang2021cade,chen2023continuous}. This approach extracts meaningful representations by distinguishing between similar and dissimilar instance pairs. It assumes that similar instances should be closer in the embedding space while dissimilar ones should be further apart~\cite{wu2018unsupervised,khosla2020supervised}. 

We implement a method based on triplet learning, focusing on the main classes—benign and malware—with a triplet loss. In our approach, a sample is considered positive if it belongs to the same class as the anchor and negative if it belongs to a different class. Unlike previous works that treat each malware family as a distinct class, leading to \( m+1 \) classes where \( m \) is the number of malware families, our method only considers the binary case. This is more annotation-friendly, as it does not require separate malware family annotation.

The learning process combines a supervised binary cross-entropy loss and a triplet margin loss. The binary cross-entropy loss is defined as:

\[
\mathcal{L}_{\text{bce}} = -\frac{1}{N} \sum_{i=1}^{N} \left[ y_i \log(\hat{y}_i) + (1-y_i) \log(1-\hat{y}_i) \right]
\]

where \( y_i \) is the true label and \( \hat{y}_i \) is the predicted probability.

The triplet margin loss is given by:

\[
\begin{aligned}
\mathcal{L}_{\text{triplet}} = \frac{1}{N} \sum_{i=1}^{N} \max\Big(0, \ 
& \|\text{enc}(x_i^a) - \text{enc}(x_i^p)\|_2^2 \\
& - \|\text{enc}(x_i^a) - \text{enc}(x_i^n)\|_2^2 + m \Big)
\end{aligned}
\]

where \(x_i^a, x_i^p, x_i^n\) are the anchor, positive, and negative samples respectively, \(\text{enc}(\cdot)\) is the encoder function, and \(m\) is the margin parameter.

The combined loss function is:

\[
\mathcal{L} = \lambda \cdot \mathcal{L}_{\text{bce}} +  \mathcal{L}_{\text{triplet}}
\]

where \(\lambda\) is a weight parameter balancing the two loss components.

















\item \textbf{Hierarchical Contrastive Classifier (HCC):} ~\cite{chen2023continuous} introduced an enhanced supervised contrastive classifier featuring a hierarchical contrastive loss function. The core idea is to ensure that samples from the same malware family are more similar than those from different families in the feature embedding space. Using an encoder network \( \text{enc} \), the embeddings of two benign or two malicious samples from different families should satisfy \( \|\text{enc}(x_1) - \text{enc}(x_2)\|_2 \leq m \). For samples from the same malware family, the embeddings should be even more tightly constrained, while embeddings of one malicious and one benign sample should be highly dissimilar, \( \|\text{enc}(x_1) - \text{enc}(x_2)\|_2 \geq 2m \).

Let \( d_{ij} \) denote the Euclidean distance between two samples \( i \) and \( j \) in the embedding space, defined as \( d_{ij} = \|\text{enc}(x_i) - \text{enc}(x_j)\|_2 \). The hierarchical contrastive loss is:

\[
\begin{aligned}
\mathcal{L}_{hc}(i) = & \frac{1}{|P(i, y_i, y_i')|} \sum_{j \in P(i, y_i, y_i')} \max(0, d_{ij} - m) \\
& + \frac{1}{|P_z(i, y_i, y_i')|} \sum_{j \in P_z(i, y_i, y_i')} d_{ij} \\
& + \frac{1}{|N(i, y_i)|} \sum_{j \in N(i, y_i)} \max(0, 2m - d_{ij})
\end{aligned}
\]

The first term ensures positive pairs, such as (benign, benign) or (malicious, malicious), are close but not overly constrained, penalizing distances only if they exceed \( m \). The second term enforces similarity within the same malware family. The last term aims to separate benign and malicious samples by at least \( 2m \).

Like the SCC, this loss is combined with binary cross-entropy loss to train the model. Note that this is the only model that requires access to malware family labels to train the model. 




\end{enumerate}


\subsection{Active Learning Sample Selection Strategy} \label{sec-al-sample}
Active learning aims to improve model performance with minimal labeled data by selectively choosing the most informative samples from a large pool of unlabeled data~\cite{ren2021survey}. For all models except HCC, we adopt the baseline uncertainty sampling strategy~\cite{DBLP:conf/sigir/LewisG94}. The key idea of uncertainty sampling is to select samples for which the model is least confident. For our models, this involves computing \(1 - \text{probability}\) (e.g., the softmax output for neural networks) for binary classes and selecting samples with the highest uncertainty.

For HCC, we employ the pseudo-label sample selection method described in~\cite{chen2023continuous}. This approach uses pseudo-labels as ground truth to compute the loss function. It calculates the pseudo-loss for contrastive learning by comparing the embeddings of test samples with those of nearby samples in the training dataset. The method then combines this contrastive loss with the binary cross-entropy loss, similar to the loss function used during training, to identify the most uncertain samples.





\begin{table*}[ht]
\centering
\caption{Performance comparison of different models on the Drebin dataset for offline learning. The results represent the mean and standard deviation over five runs with different random seeds. The best-performing model is underlined.}

\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{3.25pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc} 
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{Merged Training}} & \multicolumn{6}{c}{\textbf{Holdout Training}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c|}{\textbf{Duplicated}} & \multicolumn{3}{c|}{\textbf{Deduplicated}} & \multicolumn{3}{c|}{\textbf{Duplicated}} & \multicolumn{3}{c}{\textbf{Deduplicated}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR \\
\midrule
RF & 46.7±0.99 & \underline{0.14±0.00} & 66.8±0.74 & 41.5±0.30 & \underline{0.08±0.00} & 72.5±0.25 & 39.4±1.31 & \underline{0.16±0.03} & 72.4±1.03 & 33.2±1.01 & \underline{0.14±0.04} & 78.7±0.71 \\ 
SVM & 63.6±0.00 & 0.80±0.00 & 47.0±0.00 & 46.6±0.00 & 0.60±0.00 & 65.6±0.00 & 47.2±0.00 & 0.92±0.00 & \underline{63.2±0.00} & 33.8±0.00 & 0.70±0.00 & 76.7±0.00 \\ 
XGBoost & 63.7±2.45 & 0.18±0.01 & 48.9±2.80 & \underline{59.5±0.46} & 0.39±0.02 & 52.1±0.59 & \underline{45.2±1.92} & 0.24±0.04 & 67.3±2.01 & \underline{47.3±0.78} & 0.73±0.02 & \underline{63.4±0.66} \\ 
MLP & 66.2±3.69 & 0.41±0.08 & 45.8±4.10 & 53.6±2.08 & 0.39±0.08 & 59.5±2.12 & 44.3±2.07 & 0.87±0.06 & 66.7±1.72 & 40.9±1.05 & 0.57±0.04 & 69.8±0.82 \\ 
SCC & \underline{74.7±0.78} & 0.53±0.09 & \underline{35.0±1.51} & 57.4±0.44 & 0.63±0.25 & 53.7±2.11 & 45.6±1.18 & 0.70±0.11 & 65.7±1.35 & 37.3±0.26 & 0.63±0.10 & 73.0±0.61 \\ 
HCC & 68.4±1.73 & 0.82±0.21 & 41.3±2.52 & 56.7±0.79 & 1.04±0.12 & \underline{50.5±0.76} & 44.9±1.60 & 0.77±0.11 & 66.2±1.60 & 35.8±0.65 & 0.84±0.15 & 73.5±1.14 \\ 
\bottomrule
\end{tabular}
}

\label{tab:res-static-drebin}
\end{table*}





\begin{table*}[ht]
\centering
\caption{Performance comparison of different models on the APIGraph Dataset for offline learning}

\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{3.25pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc} 
\toprule

\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{Merged Training}} & \multicolumn{6}{c}{\textbf{Holdout Training}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c|}{\textbf{Duplicated}} & \multicolumn{3}{c|}{\textbf{Deduplicated}} & \multicolumn{3}{c|}{\textbf{Duplicated}} & \multicolumn{3}{c}{\textbf{Deduplicated}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR \\
\midrule
RF & 64.6±1.02 & \underline{0.23±0.00} & 49.6±1.08 & 61.3±0.92 & \underline{0.50±0.03} & 51.7±0.79 & 45.3±5.22 & \underline{0.12±0.02} & 68.5±4.50 & 46.8±3.89 & \underline{0.34±0.08} & 67.0±3.76  \\ 
SVM & \underline{76.0±0.00} & 1.20±0.00 & \underline{30.7±0.00} & \underline{69.7±0.00} & 1.41±0.00 & 34.9±0.00 & \underline{74.5±0.00} & 0.86±0.00 & \underline{34.7±0.00} & \underline{66.3±0.00} & 1.42±0.00 & \underline{39.5±0.00}  \\ 
XGBoost & 74.6±0.47 & 1.21±0.09 & 32.5±0.49 & 69.0±0.45 & 1.61±0.03 & \underline{34.3±0.57} & 69.5±1.40 & 1.03±0.06 & 40.2±1.65 & 65.2±0.62 & 1.33±0.05 & 41.6±0.88  \\ 
MLP & 68.6±2.28 & 0.85±0.26 & 41.9±3.77 & 63.0±2.73 & 0.96±0.37 & 46.32±4.9 & 55.6±4.26 & 0.90±0.20 & 56.2±4.85 & 57.0±3.52 & 1.67±0.64 & 49.9±6.78  \\ 
SCC & 66.1±2.79 & 1.06±0.26 & 43.8±3.94 & 66.2±2.09 & 2.11±0.57 & 35.2±1.98 & 70.36±2.9 & 1.79±0.16 & 35.3±3.33 & 57.0±3.52 & 1.67±0.64 & 49.9±6.78  \\ 
HCC & 73.3±2.37 & 1.35±0.15 & 33.3±3.90 & 66.0±1.75 & 0.92±0.17 & 42.8±2.66 & 64.2±5.17 & 1.60±0.20 & 43.8±6.61 & 62.6±2.74 & 1.59±0.26 & 43.8±4.13 \\ 
\bottomrule
\end{tabular}
}

\label{tab:res-static-apigraph}
\end{table*}








\subsection{Hyperparameter Tuning}\label{sec-hopt}

We perform hyperparameter tuning independently for two experimental setups: offline learning and continuous active learning.

In the offline learning setup, each model is trained once on the training dataset, with the validation set used to determine the optimal hyperparameters. We employ random search~\cite{bergstra2012random} for hyperparameter tuning, allocating a fixed budget of 200 searches per model on the validation set. This ensures a fair comparison across models and accounts for performance variations due to differing hyperparameter search spaces. We also perform hyperparameter tuning separately for the duplicated and deduplicated datasets.

In the continuous active learning setup, we adopt the strategy outlined in~\cite{chen2023continuous}. The validation data is divided into six-month intervals. We retrain the model using active learning for each interval and evaluate it in the subsequent month. Most hyperparameters, such as batch size for neural networks, remain consistent across the initial training and subsequent retraining phases (a total of five retraining phases, as no retraining is required for the final validation month). However, specific parameters, such as the number of training epochs during retraining, may vary. For continuous active learning hyperparameter tuning, we use random search with 100 searches per model and a fixed annotation budget of 50 samples per month, following~\cite{chen2023continuous}.

Details of the hyperparameters are provided in Appendix~\ref{appendix-hpo}.










\subsection{Evaluation Metric}

After hyperparameter tuning, we evaluate the models on the test set. The continuous active learning setup includes retraining the model each test month and evaluating it the following month. We use the same performance metrics as in~\cite{chen2023continuous}: average F1-score, False Positive Rate (FPR), and False Negative Rate (FNR). We evaluate all models on the test set using optimal hyperparameters and five different random seeds, reporting the mean and standard deviation of the metrics. It is worth noting that SVM produces deterministic results across seeds, as it uses the same training dataset without any stochastic elements. 


%These metrics differ slightly from the Area Under Time (AUT) metric in~\cite{pendlebury2019tesseract} but are highly correlated since the interval is consistently one month. Thus, conclusions from both metrics are similar.

% Four models, including the random forest and the three neural networks (MLP, SCC, HCC), depend on random seeds for initialization. This reliance makes reproducibility challenging when reimplementing on different platforms, even with identical hyperparameters~\cite{zhuang2022randomness}. To mitigate this issue, we conduct experiments using optimal hyperparameters on the test set with five different seeds, reporting the mean and standard deviation of the metrics. This approach highlights the variability in reproducing model performance across different environments. 

% While XGBoost can introduce randomness through its sampling methods, we use default parameter values (i.e., 1) to ensure deterministic outcomes for the same model parameters~\cite{xgboost_issue_2636}. We confirm deterministic results by running experiments on a different system with the same XGBoost library version.


\subsection{Experimental Settings}
We summarize the different experimental settings used in our analysis:

\begin{enumerate}
\item \textbf{Learning Settings:}
\begin{itemize}
    \item \textit{Offline learning}: The model is trained once.
    \item \textit{Active learning}: The model is retrained monthly with a fixed annotation budget. For RF, SVM, and XGBoost, we train from scratch, while for neural networks, we continue fine-tuning the previous model, following recommendations from~\cite{chen2023continuous}.
\end{itemize}

    \item \textbf{Duplicates:} 
    \begin{itemize}
        \item \textit{Duplicated}: We use the original datasets containing duplicated samples in the train, validation, and test splits.
        \item \textit{Deduplicated}: We deduplicate the datasets following the procedures in Section~\ref{sec-dedup} before conducting the experiments.
    \end{itemize}

    \item \textbf{Delayed Evaluation:} Based on whether validation data is merged with training data after hyperparameter tuning(\ref{sec-delayed}):
    \begin{itemize}
        \item \textit{Merged Training}: Merge validation data with training data before evaluating the model on test data.
        \item \textit{Holdout Training}: Train the model using only training data.
    \end{itemize}
    Both settings share the same set of hyperparameters.

\item \textbf{Active Learning Budget:} We evaluate two monthly annotation budgets for the active learning setup: 50 and 100 samples. Both settings use the model optimized with a 50-sample budget for hyperparameter tuning.

\end{enumerate}







==> sections-old/introduction.tex <==
\section{Introduction}

 
The proliferation of Android malware continues to pose significant security threats, making timely detection and mitigation critical. Machine learning (ML), particularly leveraging static analysis features, remains widely adopted in security practice due to its scalability, speed, and suitability for rapidly screening large numbers of applications~\cite{arp2014drebin, mclaughlin2017deep, mamadroid,gopinath2023comprehensive}. ML models learn patterns from data, adapt to new threats, and scale far beyond the capabilities of traditional signature-based systems. However, recent research underscores critical limitations in their reliability, reproducibility, and security assurance~\cite {arp2022and}, leading to claims that cannot be reliably corroborated. Key issues, as observed in prior works~\cite{arp2022and, flood2024bad, verma2019data}, include sampling bias, incorrect labels, data snooping, inappropriate threat models, and unsuitable baselines. This lack of rigor in the design and evaluation process undermines the validity of many reported findings ~\cite{olszewski2023get}. Such discrepancies seriously question the reliability of ML-based malware detection when deployed in operational security settings.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/hcc-code-best-worst-F1.png}    \includegraphics[width=0.35\textwidth]{figures/hcc-code-best-worst-FNR.png}
    \caption{Performance comparison of the best and worst performing neural network models for Android malware detection using the state-of-the-art continuous active learning method from~\cite{chen2023continuous}. Top: F1-score. Bottom: False Negative Rate (FNR). Models were initialized with 5 different random seeds. The average F1-score over months differs by 10.6\%, and the False Negative Rate (FNR) differs by 13.9\% between the two models, despite using the same hyperparameters. This highlights reproducibility challenges in machine learning research for Android malware detection.}
    \label{fig:hcc-best-worst}
\end{figure}

\textbf{Motivation}. We showcase an example that highlights how reliably reproducing prior results in Android malware detection can be fraught with challenges, which, if not adequately addressed, can hinder progress in this research field. See Figure~\ref{fig:hcc-best-worst}, where we examine the reproducibility of results reported by~\cite{chen2023continuous} for Android malware detection using continuous active learning. Reproduced experiments include artifacts provided by the authors, including code and datasets, and the author-provided best set of hyperparameters for the Drebin-based dataset~\cite{arp2014drebin}. We used five different random seeds and then compared the best and worst-performing models on the test set. Best model achieved an average F1 score of 79.26\% over the test months, while the worst model scored 68.65\%, indicating a performance difference of 10.6\% solely due to variations in random seed initialization.

In this paper, we study these security-critical evaluation issues by systematically studying Android malware detection methodologies. We examine three prevalent reproducibility pitfalls, including (1) data duplication, which artificially inflates model performance; (2) inadequate hyperparameter tuning, causing unfair baseline comparisons; and (3) performance instability due to variance from random model initialization. We systematically discuss how these factors cause irreproducibility and propose ways to mitigate them. We use two widely-recognized Android malware datasets, Drebin~\cite{arp2014drebin} and APIGraph~\cite{zhang2020enhancing}, and six different models, including Random Forest~\cite{breiman2001random}, Support Vector Machine~\cite{arp2014drebin}, eXtreme Gradient Boosting~\cite{chen2016xgboost}, Multilayer Perceptron~\cite{rumelhart1986learning}, Supervised Contrastive Classifier~\cite{yang2021cade}, and Hierarchical Contrastive Classifier~\cite{chen2023continuous}, previously used in Android malware analysis. We conduct comprehensive experiments under realistic offline learning, where the model is trained once, and continuous active learning, where the model is periodically retrained with a subset of annotated samples. We perform detailed model selection and hyperparameter tuning for all models in both settings. While we primarily focus on state-of-the-art continuous active learning methods~\cite{chen2023continuous}, we expand the scope by using diverse experimental settings and addressing general reproducibility issues in Android malware detection.
Contrary to common perceptions that sophisticated neural architectures inherently outperform simpler models, our results demonstrate that simpler, well-tuned tree-based methods, particularly XGBoost, frequently provide superior robustness, especially after removing dataset duplicates. These findings emphasize the need for security researchers to prioritize rigorous, reproducible evaluation methodologies over mere model complexity.


%While we focus on Android malware detection, insights from this work can be extended to other domains, such as Windows malware detection~\cite{anderson2018ember,yang2021bodmas}, and other security applications, like network intrusion detection~\cite{flood2024bad,olszewski2023get}.


\textbf{Key Contributions:}
\begin{enumerate}
    \item We systematically identify critical reproducibility issues in datasets and evaluation methods commonly used in Android malware detection, and propose rigorous methodological solutions to improve result reliability and enable fairer comparisons across models.
    \item Through comprehensive experiments on two standard datasets in both offline and continuous active learning scenarios, we demonstrate that simpler, well-tuned models (e.g., XGBoost) consistently outperform complex neural networks, challenging common assumptions in security literature.
    \item We release our extensively validated, extensible evaluation framework as open-source\footnote{\href{https://anonymous.4open.science/r/maldetect-DEC9/README.md}{https://anonymous.4open.science/r/maldetect2025}}, facilitating transparent, reproducible, and security-focused malware detection research.

\end{enumerate}









==> sections-old/limitations.tex <==
\section{Limitations \& Discussions}
\label{sec:limitations}


\subsection{Limitations}
In our study, we define duplicates as instances with identical feature inputs to the model. However, this does not necessarily correspond to true duplicates in the input space due to factors such as obfuscation, packing, feature space drift, and other complications~\cite{o2011obfuscation,yang2015appspear,chen2023overkill}. Deduplicating malware is, therefore, a challenging task and is not the primary focus of our work. Instead, our objective is to evaluate the reproducibility of reported results when using identical feature sets and machine learning models. It is important to exercise caution when interpreting these results. For example, one feature set may treat near-duplicate malware as identical, while another feature set may introduce variability between them. However, this variability is a property of the feature extraction process, distinct from the machine learning model. Consequently, we argue that deduplication is necessary when comparing different machine learning models on the same datasets, or at the very least, the variance in performance should be explicitly addressed.



Our study examined two datasets with static feature sets, although other feature sets and datasets have been proposed in the Android malware detection literature~\cite{liu2020review}. While dynamic analysis may be required for more robust malware detection, our findings regarding model selection, robust baselines, and evaluation strategies apply to other feature sets and can inform future research. Although duplicates and deduplication processes may vary across feature sets, the broader implications of our analysis remain relevant.

Datasets with labels aggregated from sources such as VirusTotal may suffer from issues related to ground truth annotations, as highlighted in prior studies~\cite{aghakhani2020malware}. However, addressing these issues is beyond the scope of our study. Our focus is on offline and continuous active learning for malware detection. In the continuous learning setting, we retrain the model monthly with new samples, as done in prior work. However, this approach may be inefficient if the model's performance has not degraded. In such cases, a drift detection mechanism may be necessary to determine when retraining is required~\cite{jordaney2017transcend}. 





\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/time (3).pdf}
    \caption{Inference time (in seconds) of different machine learning models on the Drebin (left) and APIGraph (right) datasets.}
    \label{fig:time}
\end{figure}



\subsection{Computation Time}
\label{sec:computation-time}

Figure~\ref{fig:time} illustrates a comparison of the aggregate inference times for various machine learning models evaluated on the Drebin and APIGraph test datasets. The results show that neural models consistently incur higher inference latency compared to traditional models such as Random Forest (RF) and Support Vector Machine (SVM). The experiments were conducted using Python~3.11.6 on Red Hat Enterprise Linux~9.4, running on an Intel Xeon Gold CPU at 2.20\,GHz. 




\subsection{Number of Trials and Performance Convergence}

We employ random search for hyperparameter tuning because it is the standard practice in the domain generalization literature, where training and test datasets do not adhere to the i.i.d. assumption~\cite{domainbed,yu2024rethinking}. The primary rationale behind this choice is to ensure a fair comparison across different methods. Unlike more exhaustive search strategies, random search prevents more complex models from gaining an unfair advantage simply due to a larger hyperparameter space. To maintain rigor, we set the number of trials sufficiently high to ensure that all the models we considered reached stable performance on the validation set.


We analyze model performance on the validation set as the number of hyperparameter search trials increases across different datasets. Figure~\ref{fig:offline-hpo} presents results for the offline learning setting, while Figure~\ref{fig:al-hpo} shows results for continuous active learning. Most models converge within 100 trials in offline learning, whereas convergence occurs even earlier in continuous learning, indicating that initial hyperparameters have less impact. Although validation performance generally reflects model effectiveness, this is not always the case. For instance, the RF model performs significantly better on the validation set than on the test set for the Drebin dataset in both settings.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/offline-hpo-trials.png} 

    \caption{Performance on validation set as number of hyperparameter trials is increased for offline learning}
    \label{fig:offline-hpo}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/al-hpo-trials.png} 

    \caption{Performance on validation set as number of hyperparameter trials is increased for continuous active learning}
    \label{fig:al-hpo}
\end{figure}




% \section{Influence of Individual Hyperparameters}
% Figure~\ref{fig:xgboost-hpo} illustrates the impact of individual hyperparameters
% on the validation set performance for the XGBoost model in
% the offline learning setting.




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.7\columnwidth]{figures/xgboost-all-hpo.png} 

%     \caption{Influence of individual hyperparameters on different
% datasets for XGBoost}
%     \label{fig:xgboost-hpo}
% \end{figure}












==> sections-old/pitfalls.tex <==

\begin{figure*}[t] 
\centering
\begin{subfigure}{0.47\textwidth} 
    \includegraphics[width=\textwidth]{figures/drebin-cross-split.png} 
    \caption{Drebin: Offline learning deduplication}
    \label{fig:image1}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
    \includegraphics[width=\textwidth]{figures/drebin-intra-split.png}
    \caption{Drebin: Continuous active learning deduplication}
    \label{fig:image2}
\end{subfigure}

\vspace{-0pt}  % Adjust vertical space between rows 

\begin{subfigure}{0.47\textwidth}
    \includegraphics[width=\textwidth]{figures/apigraph-cross-split.png}
    \caption{APIGraph: Offline learning deduplication}
    \label{fig:image3}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
    \includegraphics[width=\textwidth]{figures/apigraph-intra-split.png}
    \caption{APIGraph: Continuous active learning deduplication}
    \label{fig:image4}
\end{subfigure}

\caption{Fraction of unique samples retained after the deduplication process}
\label{fig:duplicates}
\end{figure*}


\section{Pitfalls in Reproducibility and Evaluation}\label{sec:pitfalls}
We critically examine key methodological and dataset-related pitfalls prevalent in existing Android malware detection research. These pitfalls can severely undermine reproducibility and practical security effectiveness, and we propose systematic strategies to mitigate their impact.

\subsection{Dataset Duplication} 
Issues of duplicates in Android malware datasets have been reported in prior studies~\cite{irolla2018duplication,zhao2021impact}. The study by~\cite{irolla2018duplication} analyzed duplicates in the original Drebin dataset~\cite{arp2014drebin} using opcode sequences and found that 50.65\% of malware samples were unique, with the rest being duplicates. They demonstrated that removing duplicates can alter the performance rankings of different machine learning models. \cite{zhao2021impact} examined duplicates in four malware datasets using APK, DEX, opcode sequences, and API calls to identify them. They also evaluated the impact of duplicates on multiple machine-learning models.

Our study differs from prior works in key ways. First, we are the first to address the reproducibility of reported results in this context. Second, we provide a time-aware analysis of duplicates' effects on malware detection models, as global metrics (e.g., F1-score) may miss monthly variations~\cite{pendlebury2019tesseract}. Lastly, unlike prior studies focused only on offline learning, we assess duplicates' impact in offline and continuous learning settings, which require different deduplication approaches, as discussed later.


\subsubsection{Defining Duplicates}

We define duplicates based strictly on feature-vector equality, meaning two samples are duplicates if their extracted feature vectors are identical. Specifically, two samples \( X \) and \( Z \) are considered duplicates if \( x_1 = z_1, x_2 = z_2, \ldots, x_n = z_n \) for an \( n \)-dimensional feature vector:
\[
X = (x_1, x_2, \ldots, x_n), \quad Z = (z_1, z_2, \ldots, z_n)
\]
This definition directly reflects the model’s perspective, differing from prior approaches relying on raw or opcode-based duplication checks~\cite{irolla2018duplication,zhao2021impact}. %By focusing on feature-space duplicates, we aim to analyze how duplicates influence the reproducibility of results for machine learning models trained on identical feature sets. 
Notably, despite using this feature-space definition, we observe a similar percentage of duplicates in the datasets as reported in prior studies. Also, detecting accurate duplicates is particularly challenging in malware analysis, which we further discuss in Section~\ref{sec:limitations}.



\subsubsection{Deduplication} \label{sec-dedup}

The process of \textit{deduplication} ensures that the dataset contains unique samples. We establish rigorous deduplication protocols based on different experimental settings in our study:

\textbf{Offline Learning Deduplication:} Here, the model is trained once on a training set and evaluated on validation and test sets. Deduplication involves selecting unique samples within and across data splits. Since the model is evaluated monthly, two levels of deduplication are required. \textit{First}, we remove samples that appear in earlier data splits: duplicates in the validation set are removed if present in the training set, while the test set excludes duplicates from both the training and validation sets. \textit{Second}, within each split, only the earliest occurrence of a sample is retained based on its appearance time. %This process ensures that all samples across the training, validation, and test sets are unique while preserving the earliest unique samples.

\textbf{Continuous Active Learning Deduplication:} Here, the definition of duplicates evolves due to monthly model retraining and changes in behavior, such as catastrophic forgetting~\cite{rahman2022limitations}. Duplicate samples are first removed from the training split, following the same approach as offline learning. For the validation and test sets, duplicates are removed only within the same month, not across different months. This allows duplicates to appear in multiple months of the test set while ensuring that each month contains unique instances. This approach is crucial for continuous learning, as periodic retraining requires the model to recognize recurring samples accurately.


\subsubsection{Duplicate Statistics in the Datasets}

Figure~\ref{fig:duplicates} illustrates the proportion of unique samples in the datasets after the deduplication process in both experimental settings. Ideally, this fraction would be 1 for both malware and benign apps, indicating no duplicates. However, our analysis shows that many duplicates are present, with varying degrees across different splits. Notably, around 50\% of the training set for the Drebin and APIGraph datasets consists of duplicate samples in benign and malware categories.

We observe two key patterns regarding duplicates in the validation and test sets. First, the fraction of duplicate samples varies monthly. Second, malware samples tend to contain more duplicates than benign samples, with certain months particularly affected. For instance, in the first test month of the Drebin dataset (July 2020), only 6.30\% of malware samples are unique in the offline-learning setting, and 9.96\% are unique in the continuous-learning setting. 

%We demonstrate in Sections~\ref{sec-offline-res} and~\ref{sec-active-res} how the presence of duplicates can undermine the replicability of reported results in Android malware detection, leading to biased evaluations of model performance.



\subsection{Inadequate Model Selection and Tuning}

A common approach for evaluating machine learning models involves splitting the dataset into training, validation, and test sets. The validation set is essential for model selection and hyperparameter tuning to prevent biased parameter choices~\cite{arp2022and}. However, previous research on Android malware detection often omits a separate validation set, leading to incomplete evaluations~\cite{arp2022and}. Our study adopts the same train, validation, and test split as in~\cite{chen2023continuous} for offline and continuous learning settings.

Another common issue is the inadequate tuning of baseline methods~\cite{arp2022and}. This often results in insufficient hyperparameter tuning for simpler models compared to more complex ones. For example, prior research has shown that appropriately tuned tree-based methods frequently outperform deep neural networks on tabular datasets~\cite{grinsztajn2022tree,mcelfresh2024neural}, even though neural networks excel in tasks like computer vision and natural language processing~\cite{DBLP:conf/nips/KrizhevskySH12,he2016deep,DBLP:conf/nips/VaswaniSPUJGKP17,DBLP:conf/naacl/DevlinCLT19}.

In Android malware detection, various models have been used in literature, such as support vector machines (SVM), random forests, gradient-boosted decision trees, and deep neural networks~\cite{arp2014drebin,mamadroid,pendlebury2019tesseract,zhang2020enhancing,chen2023continuous}. However, these models might not have been adequately calibrated due to the absence of a validation set or insufficient hyperparameter searches. Our analysis emphasizes extensive hyperparameter searches across different baseline methods, ensuring the same hyperparameter budget is allocated to each model. This approach enables a fair comparison between models and aligns with the established norms in the domain generalization literature in machine learning~\cite{domainbed}.


%We detail our procedure in Section~\ref{sec-hopt} and show how it can lead to significantly different conclusions about model performance in Section~\ref{sec-hpotxsboost}.




\subsection{Accounting for Variance from Random Initialization}

Some machine learning models, particularly neural networks, exhibit additional stochasticity independent of their hyperparameters. Their sensitivity to initial random weight initialization can lead to variations in results that depend on the training system rather than the model parameters~\cite{bouthillier2021accounting,picard2021torch}. It is common practice in the deep learning community to evaluate performance across multiple random seeds on the test set and report the average~\cite{bouthillier2020survey} to address this. However, prior studies on Android malware detection often neglect this variation, leading to irreproducible outcomes when experiments are conducted with different random seeds. We explore this issue in detail in Section~\ref{sec-offline-variance}.



\subsection{Delayed Evaluation of Models} \label{sec-delayed}

Splitting the dataset into non-overlapping temporal train, validation, and test sets facilitates better model selection. However, this approach introduces a delay between the training and test datasets. While this delay is not problematic for classical supervised learning, which assumes an independent and identically distributed setting, it poses challenges for malware detection. For example, in our study and in~\cite{chen2023continuous}, there is a six-month gap between the training and test datasets. Directly evaluating the test set using a model trained solely on the training data may not accurately reflect practical deployment scenarios. Ideally, the model should be trained with more recent data before deployment~\cite{arp2022and}.

To address this, we merge the training and validation datasets after hyperparameter tuning and evaluate the model on the test dataset. We propose that this approach provides a fairer estimate of model performance in offline learning, where the model is inherently delayed by the time the test month begins. Merging validation data with training data is a common practice in temporal domain generalization~\cite{yao2022wild}. We refer to this as the \textbf{Merged Training} setup, in contrast to the \textbf{Holdout Training} setup, where the model is trained only on the training dataset and evaluated on the test dataset. The impact of these two evaluation settings is demonstrated in Sections~\ref{sec-offline-res} and~\ref{sec-active-res}.





==> sections-old/recommendations.tex <==
% \section{Recommendations for Better Reproducibility}

% Based on our reproducibility study of Android malware detection, we propose a set of recommendations to enhance the reproducibility of reported results. These recommendations should be used alongside existing guidelines for machine learning in security~\cite{arp2022and,olszewski2023get} and Android malware detection~\cite{pendlebury2019tesseract} to improve reproducibility in future work.

% \begin{itemize}
%     \item Datasets should be deduplicated to provide a more accurate estimation of model performance and improve the reproducibility of research.
%     \item Datasets should be split into non-overlapping train, validation, and test sets for model selection and hyperparameter tuning. Once tuning is complete, the validation set should be merged with the training data in offline learning settings to estimate model performance on test data.
%     \item Proper hyperparameter tuning for baseline machine learning models is crucial to understanding improvements introduced by novel approaches. For Android malware detection, XGBoost is a strong benchmark for offline and active learning settings.
%     \item For neural networks, reporting performance using multiple random seeds on the test set is important to account for variance introduced by random weight initialization.
%     \item Instead of relying on a single metric, a thorough analysis should be performed on month-by-month results to compare different models and identify any potential bias leading to a flawed conclusion.
% \end{itemize}

==> sections-old/results.tex <==








\begin{figure*}
\centering
    \includegraphics[width=0.49\textwidth]{figures/apigraph-dedup-f1.png}
    \includegraphics[width=0.49\textwidth]{figures/apigraph-dup-f1.png}
    \caption{F1-score over the test months on the APIGraph for (left) deduplicated (right) duplicated datasets}
    \label{fig:var-apigraph}
\end{figure*}


\begin{figure*}
\centering
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figures/drebin-dedup-f1.png}
    \caption{F1-score on deduplicated data}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figures/drebin-dup-f1.png}
    \caption{F1-score on duplicated dataset}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figures/drebin-dup-fnr.png}
    \caption{FNR on duplicated dataset}
  \end{subfigure}
  
  \caption{Performance in test months on the Drebin datasets for Merged Training setting}
  \label{fig:var-drebin}
\end{figure*}


\section{Offline Learning Results \& Analysis} \label{sec-offline-res}




\subsection{Malware Detection Performance}

We present the results of six models in Table~\ref{tab:res-static-drebin} for the Drebin dataset and Table~\ref{tab:res-static-apigraph} for the APIGraph dataset. These results encompass the various experimental settings discussed previously. Key findings are summarized as follows:

\begin{enumerate}
    \item \textbf{Impact of duplicates on model performance:} Deduplicated datasets generally perform worse than those with duplicates, indicating that duplicates may inflate performance metrics. For instance, in the Drebin dataset's merged training setting, the F1-score differences for the SVM and SCC models are 17.0 and 17.3, respectively, between duplicate and deduplicated datasets.

    \item \textbf{Benefits of merged training:} Merging validation data with training data before final evaluation consistently enhances performance. In the Drebin deduplicated dataset, the average F1-score improvement ranges from 8.3 (RF) to 20.9 (HCC), demonstrating the benefits of additional training data and its alignment with practical applications.

    \item \textbf{Duplicates influence model preference:} Duplicates can skew model comparisons. For example, in the Drebin dataset merge-training setting, SCC outperforms XGBoost by 11 in average F1-score. However, after deduplication, XGBoost outperforms SCC by 2.1 in average F1-score.

    \item \textbf{XGBoost as a strong baseline on deduplicated datasets:} 
With proper tuning, XGBoost achieves the highest average F1-score on the deduplicated Drebin dataset and remains competitive on APIGraph, highlighting its effectiveness as a baseline model. In contrast, while SVM performs well on APIGraph, its performance drops significantly on the Drebin dataset after deduplication.

    % \item \textbf{Increased Variability Due to Duplicates:} Models reliant on random initialization (RF, MLP, SCC, HCC) exhibit greater performance variance on duplicate datasets in most experimental settings. Duplicates not only inflate results but also increase variability, affecting reproducibility. For the APIGraph dataset in the duplicate holdout training setting, HCC's average F1-score ranges from 57.7 to 70.7, showing a 13-point difference due to random seed variations. We discuss this issue further below.
\end{enumerate}








\begin{figure*}
  \centering  \includegraphics[width=0.45\textwidth]{figures/apigraph-2015-11.png}    \includegraphics[width=0.45\textwidth]{figures/drebin-2021-01.png}
    \caption{Frequency of Unique and top-10 Duplicate malware samples for the month 2015-11 on the APIGraph dataset (left) and the month 2021-01 on the Drebin dataset (right)}
    \label{fig:dupe-sample}
\end{figure*}









\subsection{Duplicates and Variance in Performance} \label{sec-offline-variance}

Figures~\ref{fig:var-apigraph} and \ref{fig:var-drebin} show the month-by-month performance of four models (SVM, XGBoost, MLP, HCC) on the APIGraph and Drebin datasets under the merged training setting for both duplicated and deduplicated datasets. Key conclusions from the results are:

\begin{enumerate}
    \item \textbf{Impact of duplicates on performance trends:} On both datasets, models generally exhibit a downward performance trend over time due to concept drift. However, this trend is less evident in the original datasets with duplicates, where sudden fluctuations occur. For example, all models experienced a performance drop in November 2015 on the APIGraph dataset, explained by duplicate inputs, as shown in Figure~\ref{fig:dupe-sample} (left). Of the 488 malware samples that month, 190 have identical input features. If a model fails to detect one correctly, it fails for all, resulting in a significant performance drop.

    \item \textbf{High variance due to duplicates:} As seen in Figure~\ref{fig:var-drebin}(b), duplicates can cause high variance in model performance. Figure~\ref{fig:var-drebin}(c) shows that this effect is primarily due to variance introduced by false negative rates (FNRs). Figure~\ref{fig:dupe-sample}(right) illustrates the frequency of unique, and top-10 duplicated malware samples for January 2021 on the Drebin dataset. Specifically, 348 out of 385 samples are duplicates of the same input feature, resulting in significant variance for models relying on random initialization, such as neural networks. Two of five MLPs trained with different seeds achieved high F1 scores (93.7 and 94.0), while the others scored much lower (21.4, 24.6, 24.8), indicating high fluctuations due to duplicates. A theoretical classifier correctly identifying all malware samples this month has an FNR of 0. If it fails to detect this single duplicated sample, the FNR rises to 90.4\%. Conversely, a classifier detecting no samples has an FNR of 100\%, but identifying only the duplicated sample reduces the FNR to 9.6\%. This highlights the need to deduplicate datasets for models relying on random initialization to prevent performance disparities caused by different initializations.

      \item \textbf{Importance of reporting performance with multiple
seeds:} Although deduplication reduces extreme variance in model performance for certain months, neural networks can still show performance variation due to random initialization, as seen in Figure~\ref{fig:var-drebin}(a). For instance, in four test months (2021-01, 2021-08, 2021-10, 2021-12), the MLP had a standard deviation of average F1-scores greater than 5, even on the deduplicated Drebin dataset. Therefore, accounting for this randomness when reporting neural network performance is essential.
\end{enumerate}




















\subsection{Effective Model Selection for Robust Baselines} \label{sec-hpotxsboost}

Our experiments with offline learning show that the XGBoost model achieves superior performance across various experimental settings, contrasting with previous results from~\cite{chen2023continuous}. The key reason is the expanded hyperparameter search space. We included more hyperparameters and broadened the search range, as detailed in Appendix~\ref{appendix-hpo}. A critical change was the number of boosting rounds considered.\cite{chen2023continuous} tested rounds ranging from 10 to 100. However, XGBoost often benefits from more boosting rounds, particularly on the APIGraph dataset, where 400 rounds yielded the best results for duplicated and deduplicated datasets. This underscores the importance of proper hyperparameter tuning to establish stronger baseline models~\cite{arp2022and}.

Figure~\ref{fig:xgboost-round} illustrates how the number of boosting rounds affects XGBoost's performance on the validation dataset across different datasets in an offline learning setup.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/xgboost_num_boost_round.png}
    \caption{Effect of number of boosting rounds during learning for XGBoost model on different datasets}
    \label{fig:xgboost-round}
\end{figure}












\begin{table*}[]
\caption{Performance of different models on the Drebin Dataset for continuous active learning with 50 \& 100 annotation budget per month}
\centering
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{3.25pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc} 
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{Budget=50}} & \multicolumn{6}{c}{\textbf{Budget=100}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c|}{\textbf{Merged Training}} & \multicolumn{3}{c|}{\textbf{Holdout Training}} & \multicolumn{3}{c|}{\textbf{Merged Training}} & \multicolumn{3}{c}{\textbf{Holdout Training}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR \\
\midrule
RF & 61.9±0.73&\underline{0.13±0.02}&53.0±0.88&62.7±1.11&\underline{0.11±0.00}&52.4±1.11&62.8±1.24&\underline{0.13±0.01}&52.1±1.30&63.6±0.47&\underline{0.12±0.03}&51.3±0.40 \\ 
SVM &64.4±0.00&0.22±0.00&48.7±0.00&59.6±0.00&0.23±0.00&54.1±0.00&68.1±0.00&0.24±0.00&44.6±0.00&63.9±0.00&0.26±0.00&49.1±0.00 \\ 
XGBoost & \underline{82.2±0.60}&0.15±0.00&\underline{27.3±0.76}&\underline{81.1±0.15}&0.14±0.01&\underline{29.2±0.21}&\underline{82.5±0.29}&0.15±0.01&\underline{26.9±0.32}&\underline{82.5±0.45}&0.14±0.01&\underline{27.0±0.57} \\ 
MLP & 67.9±0.65&0.49±0.03&43.3±0.70&61.8±0.54&0.35±0.02&51.0±0.49&70.2±0.42&0.38±0.03&40.6±0.46&65.7±3.37&0.36±0.06&46.2±4.17 \\ 
SCC & 71.0±0.64&0.59±0.04&37.4±0.29&68.2±1.83&0.50±0.07&41.6±2.21&73.7±1.20&0.57±0.10&33.7±1.35&72.1±0.88&0.48±0.07&37.0±1.44 \\ 
HCC & 73.5±0.27 & 0.66±0.04 & 32.8±0.85 & 68.5±3.38&0.57±0.05&40.3±4.37&75.6±0.96&0.68±0.06&29.4±1.07&72.6±2.10&0.57±0.02&35.2±2.64 \\ 
\bottomrule
\end{tabular}
}

\label{tab:res-al-drebin}
\end{table*}




\begin{table*}[]
\caption{Performance of different models on the APIGraph Dataset for continuous active learning with 50 \& 100 annotation budget per month}
\centering
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{3.25pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc} 
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{Budget=50}} & \multicolumn{6}{c}{\textbf{Budget=100}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c|}{\textbf{Merged Training}} & \multicolumn{3}{c|}{\textbf{Holdout Training}} & \multicolumn{3}{c|}{\textbf{Merged Training}} & \multicolumn{3}{c}{\textbf{Holdout Training}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR & F1 & FPR & FNR \\
\midrule
RF & 87.1±0.15&\underline{0.27±0.00}&19.4±0.28&87.4±0.20&\underline{0.30±0.01}&18.6±0.34&89.0±0.11&\underline{0.26±0.01}&16.4±0.13&89.4±0.11&\underline{0.28±0.01}&15.6±0.11 \\ 
SVM &83.7±0.00&0.60±0.00&21.4±0.00&84.4±0.00&0.67±0.00&19.2±0.00&84.8±0.00&0.63±0.00&19.0±0.00&85.2±0.00&0.75±0.00&16.9±0.00 \\ 
XGBoost & \underline{88.7±0.21}&0.55±0.01&\underline{13.8±0.31}&\underline{88.9±0.11}&0.53±0.03&\underline{13.7±0.11}&\underline{90.4±0.13}&0.48±0.01&\underline{11.6±0.21}&\underline{90.6±0.18}&0.45±0.01&\underline{11.5±0.16} \\ 
MLP & 85.7±0.67&0.47±0.03&19.6±1.12&85.7±0.40&0.47±0.05&19.5±1.10&87.4±0.29&0.47±0.02&16.6±0.49&87.2±0.09&0.49±0.04&16.6±0.60 \\ 
SCC & 85.6±0.37&0.85±0.07&15.1±0.27&86.0±0.71&0.81±0.08&14.8±0.31&86.1±0.38&0.95±0.07&12.8±0.61&85.7±2.80&2.03±2.51&12.9±0.48 \\ 
HCC & 87.1±0.36&0.64±0.05&15.6±0.95&86.7±0.15&0.56±0.03&17.2±0.36&87.5±0.78&0.56±0.03&15.5±1.11&87.4±0.27&0.59±0.02&15.6±0.14 \\ 
\bottomrule
\end{tabular}
}

\label{tab:res-al-apigraph}
\end{table*}



\subsection{Duplicates \& Model Selection}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/xgboost_balance.png}
    \caption{Effect of balancing the weight of the classes during learning for XGBoost model on different datasets}
    \label{fig:xgboost-balance}
\end{figure}


The presence of duplicates can influence hyperparameter tuning and model selection. Figure~\ref{fig:xgboost-balance} demonstrates this for XGBoost by adjusting the "scale\_pos\_weight" parameter to address class imbalance. In the imbalanced setting, the malware class weight is set to 1, while in the balanced setting, it matches the benign-to-malware ratio in the training set. Balancing improves validation performance for duplicated datasets but may reduce performance on the deduplicated APIGraph dataset, suggesting that duplicates can alter hyperparameter behavior for the same model.




\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/xgboost_attr_from_dedup_to_org.pdf}
    \caption{Comparison of feature weights for the top 50 features in XGBoost models trained on the deduplicated Drebin dataset and their corresponding weights in the model trained on the original duplicated dataset.}
    \label{fig:xgboost-xai-dedup2org}
\end{figure}

Figure~\ref{fig:xgboost-xai-dedup2org} illustrates how duplicates affect feature weighting in XGBoost. It compares feature importance between models trained on the deduplicated and original duplicated Drebin datasets. The top 50 features from the deduplicated model were extracted and their importance evaluated in the duplicated model. The results show a clear disparity in feature importance distribution between the two models.


























\section{Continuous Active Learning Results \& Analysis} \label{sec-active-res}

In the continuous active learning setting, duplicates pose additional challenges beyond those in offline learning. Since active learning relies on human experts to select samples for annotation, increasing the diversity of selected samples is crucial~\cite{settles2009active}. Duplicates can lead to redundant selections, wasting the annotation budget. A simple heuristic can identify previously annotated samples and replace them with their existing annotations. Thus, using duplicated datasets in an active learning setting is impractical, and our analysis primarily focuses on deduplicated datasets.




We present the results of the six models in Tables~\ref{tab:res-al-drebin} and \ref{tab:res-al-apigraph} for the Drebin and APIGraph datasets, discussing merged and holdout training settings. Key findings are summarized below:

\begin{enumerate}
    \item \textbf{XGBoost as a strong baseline in continuous active learning:} XGBoost achieves the highest average F1 score across all experimental settings in continuous active learning. This is especially evident in the challenging Drebin dataset, where it surpasses the second-best model by 8.7\% in the merged training setting. This highlights the importance of selecting a strong baseline model and underscores XGBoost's effectiveness in Android malware detection.

    \item \textbf{Benefits of Contrastive Learning for Neural Networks:} The neural networks trained with contrastive learning, SCC, and HCC outperform baseline neural networks in all settings, indicating the effectiveness of contrastive learning in enhancing robustness to concept drift. HCC further outperforms SCC, demonstrating the advantages of hierarchical contrastive learning and the pseudo-loss sample selector introduced in~\cite{chen2023continuous}. However, more improvements are needed to match XGBoost's performance.

    \item \textbf{Random Forest as a Competitive Baseline on APIGraph:} Even simpler tree-based methods like Random Forest achieve competitive performance on the APIGraph dataset, often surpassing more complex neural networks. With consistently low false positives, RF is a strong candidate model for this dataset, illustrating that simpler models can compete effectively with complex ones in a compact feature space.

    \item \textbf{Performance Gains from Merged Training:} Merging the validation set with the training set can enhance performance on test data, particularly for neural networks. However, the performance difference is less pronounced than offline learning since models are retrained during validation months with a subset of samples.
\end{enumerate}









% \subsection{MLP}

% \begin{figure}
%     \includegraphics[width=0.47\textwidth]{figures/IGXAI.pdf}
%     \caption{Attribution values of top-50 features in MLP for offline learning (top) and active learning (bottom) settings}
%     \label{fig:xai-mlp}
% \end{figure}

% \textcolor{red}{Given a trained model $F$ and input $X={x_1,.......x_n}$ where $n$ is the number of test samples and each input is $d$ dimensional, a feature attribution based post-hoc explanation method $\phi(x)$ outputs a $d$ dimensional vector of attribution scores $a^d$ for the input sample $x$ (also, known as feature importance). These scores quantify the importance of each feature in the given model prediction $F(x)$. We use integrated gradient \cite{sundararajan2017axiomatic} for explanation as this method has demonstrated to perform superior than other feature attribution methods in various security applications \cite{bhusal2023sok}. We apply post-hoc explanation method to the trained Android malware detection model using MLP architecture for both offline learning and active learning. We consider the evaluation of the offline model on the test set from 2021-11 which is 12 months away from the training dataset. We utilize the active learning model trained upto the dataset with timestamp 2021-10.}

% \textcolor{red}{In Figure \ref{fig:xai-mlp}, the first plot shows the results from a model trained on older data, which does not include more recent applications. Since this model has not been updated with new data, it continues to rely on features that may have been relevant in earlier datasets but are less effective for the more modern apps appearing in 2021-11. Hence, it assigns almost zero importance to many features which could have been removed during API updates or, no loner in use by several applications. The second plot on active learning shows a more evenly spread feature attribution values for several features. This model has been exposed to more recent data and, as a result, can better adapt to the changes and trends present in apps from 2021-11. 
% }







==> sections-old/xai.tex <==


\section{Post-hoc explainability}
To examine the change in learned features over time, we conducted a comparative analysis of XGBoost and MLP classifiers on APIGraph dataset using SHAP-based explanations~\cite{lundberg2017unified}. For XGBoost and MLP based models, we first identified the union of the top-10 most important features from July 2013 and June 2014, using SHAP~\cite{lundberg2017unified} (specifically, TreeSHAP for XGBoost and KernelSHAP for MLP). We then restricted evaluation to this union set and, for every model trained monthly from July 2013 to June 2014, we recomputed feature importance using correctly classified malware samples from the same month’s test data. Feature importances were normalized to enable direct comparison. The resulting heatmaps (Figures~\ref{fig:shapxgboost} and \ref{fig:shapmlp}) illustrate how feature importance evolves over time.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{sections/fig/xgboost.pdf}
    \caption{Heatmap showing the evolution of normalized feature importance for XGBoost models from July 2013 to June 2014.}
    \label{fig:shapxgboost}
\end{figure}

Figure~\ref{fig:shapxgboost} shows that in XGBoost models multiple feature (eg. idx 12, 16 and 87) remain consistently influential. However, other features fluctuate across months, indicating model sensitivity to month-specific variations. In contrast, with MLP models, Figure~\ref{fig:shapmlp} shows a sharper dominance of individual feature (e.g. idx 16), followed by more distributed reliance on additional features. 

\textcolor{red}{does this mean, while xgboost models adapt according to monthly retraining, MLP are kind of stuck on same small set of features?}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{sections/fig/mlp.pdf}
    \caption{Heatmap showing the evolution of normalized feature importance for MLP models from July 2013 to June 2014.}
    \label{fig:shapmlp}
\end{figure}





==> sections/recommendations.tex <==
% \section{Recommendations for Better Reproducibility}

% Based on our reproducibility study of Android malware detection, we propose a set of recommendations to enhance the reproducibility of reported results. These recommendations should be used alongside existing guidelines for machine learning in security~\cite{arp2022and,olszewski2023get} and Android malware detection~\cite{pendlebury2019tesseract} to improve reproducibility in future work.

% \begin{itemize}
%     \item Datasets should be deduplicated to provide a more accurate estimation of model performance and improve the reproducibility of research.
%     \item Datasets should be split into non-overlapping train, validation, and test sets for model selection and hyperparameter tuning. Once tuning is complete, the validation set should be merged with the training data in offline learning settings to estimate model performance on test data.
%     \item Proper hyperparameter tuning for baseline machine learning models is crucial to understanding improvements introduced by novel approaches. For Android malware detection, XGBoost is a strong benchmark for offline and active learning settings.
%     \item For neural networks, reporting performance using multiple random seeds on the test set is important to account for variance introduced by random weight initialization.
%     \item Instead of relying on a single metric, a thorough analysis should be performed on month-by-month results to compare different models and identify any potential bias leading to a flawed conclusion.
% \end{itemize}
